Ground State Phase Diagram of $\text{SU}(3)$ $t$-$J$ Chain

Distinct from the $\text{SU}(2)$ case, the fermionic systems with $\text{SU}(N)$ symmetry are expected to exhibit novel physics, such as exotic singlet formation. Using the density matrix renormalization group technique, we obtain the ground state phase diagram of the $\text{SU}(3)$ $t$-$J$ chain for density $n<1$. The ground state phase diagram includes the Luttinger liquid, the extended Luther-Emery liquid characterized by a spin gap, and the phase separation state. We quantitatively assess the characteristics of the three phases by measuring spin gap, compressibility, various correlation functions and structure factors. We further study the extended Luther-Emery liquid phase and discover molecular superfluid quasi-long-range order. The mechanism of the molecular superfluid is the combination of three $\text{SU}(3)$ fermions on sites that are not completely connected. Accordingly, we can speculate the behavior of the $\text{SU}(N)$ $t$-$J$ chain model with larger $N$ values, operating within the same filling regime.

==> citename.tex <==
Possible high Tc superconductivity in the Ba−La−Cu−O system
J. G. Bednorz, K. A. Müller, Zeitschrift für Physik B Condensed Matter 64, 189 (1986). 
SPRINGER LINK

The Resonating Valence Bond State in La2CuO4 and Superconductivity
P. W. Anderson, Science 235, 1196 (1987).

Effective Hamiltonian for the superconducting Cu oxides
F. C. Zhang and T. M. Rice, Phys. Rev. B 37, 3759 (1988).

Phase Diagram of the Two-Dimensional t-J Model
M. Ogata, M. U. Luchini, S. Sorella, and F. F. Assaad, Phys. Rev. Lett. 66, 2388 (1991).

Ground-state phase diagram of the two-dimensional t-J model
A. Moreno, A. Muramatsu, and S. R. Manmana, Phys. Rev. B 83, 205113 (2011).

Ultraviolet Behavior of Non-Abelian Gauge Theories
D. J. Gross and F. Wilczek, Phys. Rev. Lett. 30, 1343 (1973).

Reliable Perturbative Results for Strong Interactions?
H. D. Politzer, Phys. Rev. Lett. 30, 1346 (1973).

Model for the metal-insulator transition in graphene superlattices and beyond
N. F. Q. Yuan and L. Fu, Phys. Rev. B 98, 045103 (2018).

Quantum simulations with ultracold quantum gases
I. Bloch, J. Dalibard, and S. Nascimbène, Nature Physics 8, 267 (2012).

Ultracold quantum gases in optical lattices
I. Bloch, Nature Physics 1, 23 (2005).

Quantum simulation of exotic Z2 topological orders with ultracold atoms
R. Zhang, Y. Cheng, P. Zhang, and H. Zhai, Nature Reviews Physics 2, 213 (2020).

Quantum simulations with trapped ions
R. Blatt and C. F. Roos, Nature Physics 8, 277 (2012).

Observation of a Fermi liquid in a highly tunable two-dimensional Fermi gas
D. Tusi et al., Nature Physics 18, 1201 (2022).

Realization of a SU(2)×SU(6) System of Fermions in a Cold Atomic Gas
S. Taie, R. Yamazaki, S. Sugawa, and Y. Takahashi, Nature Physics 8, 825 (2012).

Observation of antiferromagnetic correlations in a 1D SU(N) Hubbard model
S. Taie et al., Nature Physics 18, 1356 (2022).

Phase transitions in anisotropic SU(N) spin chains
C. Itoi, S. Qin, and I. Affleck, Phys. Rev. B 61, 6747 (2000).

Exact critical exponents for quantum spin chains
I. Affleck, Nuclear Physics B 265, 409 (1986).

Current algebra and Wess-Zumino model in two dimensions
V. Knizhnik and A. Zamolodchikov, Nuclear Physics B 247, 83 (1984).

Conformal Field Theory
P. Di Francesco, P. Mathieu, and D. Sénéchal, (Springer, New York, 1997).

Model for the Mott transition in the two-dimensional Hubbard model
B. Sutherland, Phys. Rev. B 12, 3795 (1975).

Exact diagonalization of the t-J model on small clusters
P. Nataf and F. Mila, Phys. Rev. B 93, 155134 (2016).

Dimer-dimer correlations in the two-dimensional t-J model
K. Wan, P. Nataf, and F. Mila, Phys. Rev. B 96, 115159 (2017).

Magnetic properties of the t-J model on a square lattice
D. Vörös and K. Penc, Phys. Rev. B 104, 184426 (2021).

Spin dynamics in the two-dimensional t-J model
P. Nataf and F. Mila, Phys. Rev. B 97, 134420 (2018).

Pairing in the two-dimensional t-J model
M. Führinger et al., Annalen der Physik 12, 922-936 (2008).

Competing orders in the two-dimensional t-J model
P. Fromholz et al., Phys. Rev. B 99, 054414 (2019).

Quantum criticality in the two-dimensional t-J model
S. Gozel, P. Nataf, and F. Mila, Phys. Rev. Lett. 125, 057202 (2020).

Finite-temperature properties of the two-dimensional t-J model
P. Nataf, S. Gozel, and F. Mila, Phys. Rev. B 104, L180411 (2021).

Phase diagram of the one-dimensional t-J model
S. Capponi, P. Lecheminant, and K. Totsuka, Annals of Physics 367, 50 (2016).

Quantum Physics in One Dimension
T. Giamarchi, (Clarendon; Oxford University Press, Oxford: New York, 2004).

Bosonization and Strongly Correlated Systems
*A. O. Gogolin, A. A. Nersesyan, and A. M. Tsvelik, (Cambridge
